Transductive Optimization of Top k Precision

Consider a binary classification problem in which the learner is given a labeled training set, an unlabeled test set, and is restricted to choosing exactly $k$ test points to output as positive predictions. Problems of this kind---{\it transductive precision@$k$}---arise in information retrieval, digital advertising, and reserve design for endangered species. Previous methods separate the training of the model from its use in scoring the test points. This paper introduces a new approach, Transductive Top K (TTK), that seeks to minimize the hinge loss over all training instances under the constraint that exactly $k$ test instances are predicted as positive. The paper presents two optimization methods for this challenging problem. Experiments and analysis confirm the importance of incorporating the knowledge of $k$ into the learning process. Experimental evaluations of the TTK approach show that the performance of TTK matches or exceeds existing state-of-the-art methods on 7 UCI datasets and 3 reserve design problem instances.

==> tables/old_prec_1.tex <==
heart & 270 / 13 / 0.44 & {\bf 1.000}& {\bf 0.986}& {\bf 0.986}& {\bf 1.000}& {\bf 0.971}& {\bf 1.000}& {\bf 1.000}& {\bf 1.000}\tabularnewline
australian & 690 / 14 / 0.44 & {\bf 0.982}& NaN& {\bf 0.929}& {\bf 0.976}& {\bf 0.976}& 0.959& {\bf 0.982}& {\bf 0.971}\tabularnewline
german-numer & 1000 / 24 / 0.30 & 0.696& {\bf 0.712}& 0.668& {\bf 0.720}& 0.560& 0.672& {\bf 0.704}& {\bf 0.728}\tabularnewline
diabetes & 768 / 8 / 0.35 & {\bf 0.863}& {\bf 0.858}& {\bf 0.816}& {\bf 0.858}& {\bf 0.768}& 0.800& {\bf 0.853}& {\bf 0.847}\tabularnewline
breast-cancer & 683 / 9 / 0.35 & {\bf 1.000}& {\bf 1.000}& {\bf 1.000}& {\bf 1.000}& {\bf 1.000}& {\bf 1.000}& {\bf 1.000}& {\bf 1.000}\tabularnewline
ionosphere & 351 / 33 / 0.64 & 0.756& 0.689& 0.789& 0.800& {\bf 0.944}& 0.778& {\bf 0.856}& {\bf 0.900}\tabularnewline
splice & 3175 / 60 / 0.52 & {\bf 1.000}& {\bf 1.000}& {\bf 1.000}& {\bf 0.999}& {\bf 0.997}& NaN& {\bf 1.000}& {\bf 0.997}\tabularnewline
spambase & 4601 / 57 / 0.39 & {\bf 0.969}& 0.960& 0.963& {\bf 0.968}& {\bf 0.978}& NaN& {\bf 0.970}& {\bf 0.976}\tabularnewline
sonar & 208 / 60 / 0.47 & {\bf 0.960}& {\bf 0.940}& {\bf 0.920}& {\bf 0.980}& {\bf 0.960}& {\bf 1.000}& {\bf 0.980}& {\bf 1.000}\tabularnewline
svmguide3 & 1284 / 22 / 0.26 & 0.863& {\bf 0.878}& 0.831& 0.853& {\bf 0.909}& NaN& 0.841& 0.850\tabularnewline
\hline
\small AVERAGE &   & 0.909& 0.899& 0.890& 0.915& 0.907& 0.904& 0.919& {\bf 0.927}\tabularnewline


==> tables/old_prec_2.tex <==
heart & 270 / 13  /  0.44 & {\bf 0.993}& {\bf 0.986}& {\bf 0.986}& {\bf 1.000}& 0.929& {\bf 1.000}& {\bf 0.993}& {\bf 1.000}\tabularnewline
australian & 690  /  14 / 0.44 & {\bf 0.968}& NaN& {\bf 0.950}& {\bf 0.968}& 0.932& {\bf 0.968}& {\bf 0.968}& {\bf 0.968}\tabularnewline
german-numer & 1000 / 24 / 0.30 & {\bf 0.682}& {\bf 0.682}& {\bf 0.670}& {\bf 0.672}& 0.542& {\bf 0.654}& {\bf 0.680}& {\bf 0.676}\tabularnewline
diabetes & 768 / 8 / 0.35 & {\bf 0.826}& {\bf 0.805}& 0.779& {\bf 0.839}& 0.755& 0.797& {\bf 0.837}& {\bf 0.842}\tabularnewline
breast-cancer & 683 / 9 / 0.35 & {\bf 1.000}& {\bf 1.000}& {\bf 1.000}& {\bf 1.000}& {\bf 0.994}& {\bf 1.000}& {\bf 1.000}& {\bf 1.000}\tabularnewline
ionosphere & 351 / 33 / 0.64 & 0.867& 0.806& 0.856& 0.867& {\bf 0.956}& 0.861& {\bf 0.922}& {\bf 0.933}\tabularnewline
splice & 3175 / 60 / 0.52 & {\bf 0.994}& {\bf 0.995}& {\bf 0.995}& {\bf 0.992}& 0.987& NaN& {\bf 0.996}& {\bf 0.993}\tabularnewline
spambase & 4601 / 57 / 0.39 & {\bf 0.971}& 0.967& 0.968& 0.968& {\bf 0.973}& NaN& {\bf 0.973}& {\bf 0.971}\tabularnewline
sonar & 208 / 60 / 0.47 & {\bf 0.940}& 0.910& 0.880& {\bf 0.980}& 0.920& {\bf 1.000}& {\bf 0.990}& {\bf 0.980}\tabularnewline
svmguide3 & 1284 / 22 / 0.26 & {\bf 0.836}& {\bf 0.820}& 0.797& {\bf 0.836}& {\bf 0.784}& NaN& {\bf 0.831}& {\bf 0.834}\tabularnewline
\hline
\small AVERAGE &   & 0.908& 0.893& 0.888& 0.912& 0.877& 0.906& 0.919& {\bf 0.920}\tabularnewline


==> tables/res_prec_1.tex <==
S16 & 634 / 38 / 0.33 & {\bf 0.644}& {\bf 0.672}& 0.620& {\bf 0.640}& {\bf 0.652}& {\bf 0.604}& {\bf 0.672}& {\bf 0.664}\tabularnewline
S17 & 634 / 38 / 0.30 & {\bf 0.628}& {\bf 0.640}& {\bf 0.620}& {\bf 0.640}& {\bf 0.596}& 0.368& {\bf 0.640}& {\bf 0.640}\tabularnewline
S18 & 634 / 38 / 0.40 & {\bf 0.440}& {\bf 0.436}& {\bf 0.432}& {\bf 0.452}& 0.360& 0.360& {\bf 0.448}& {\bf 0.464}\tabularnewline
S19 & 634 / 38 / 0.37 & 0.568& {\bf 0.612}& {\bf 0.596}& {\bf 0.580}& {\bf 0.572}& 0.432& {\bf 0.632}& {\bf 0.624}\tabularnewline
\hline
\small AVERAGE &   & 0.570& 0.590& 0.567& 0.578& 0.545& 0.441& {\bf 0.598}& {\bf 0.598}\tabularnewline


==> tables/res_prec_2.tex <==
S16 & 634 / 38 / 0.33 & {\bf 0.631}& {\bf 0.592}& 0.604& {\bf 0.629}& {\bf 0.639}& 0.580& {\bf 0.641}& {\bf 0.629}\tabularnewline
S17 & 634 / 38 / 0.30 & {\bf 0.596}& {\bf 0.578}& {\bf 0.604}& {\bf 0.622}& 0.535& 0.429& {\bf 0.602}& {\bf 0.618}\tabularnewline
S18 & 634 / 38 / 0.40 & {\bf 0.449}& {\bf 0.435}& 0.400& 0.424& {\bf 0.398}& {\bf 0.375}& {\bf 0.447}& {\bf 0.439}\tabularnewline
S19 & 634 / 38 / 0.37 & 0.559& {\bf 0.543}& 0.533& {\bf 0.592}& {\bf 0.547}& 0.475& {\bf 0.582}& {\bf 0.584}\tabularnewline
\hline
\small AVERAGE &   & 0.559& 0.537& 0.535& 0.567& 0.530& 0.465& {\bf 0.568}& 0.568\tabularnewline

